Accelerating Recommender Model Training by Dynamically Skipping Stale Embeddings

Training recommendation models pose significant challenges regarding resource utilization and performance. Prior research has proposed an approach that categorizes embeddings into popular and non-popular classes to reduce the training time for recommendation models. We observe that, even among the popular embeddings, certain embeddings undergo rapid training and exhibit minimal subsequent variation, resulting in saturation. Consequently, updates to these embeddings lack any contribution to model quality. This paper presents Slipstream, a software framework that identifies stale embeddings on the fly and skips their updates to enhance performance. This capability enables Slipstream to achieve substantial speedup, optimize CPU-GPU bandwidth usage, and eliminate unnecessary memory access. SlipStream showcases training time reductions of 2x, 2.4x, 1.2x, and 1.175x across real-world datasets and configurations, compared to Baseline XDL, Intel-optimized DRLM, FAE, and Hotline, respectively.

==> body/tables/algo_example.tex <==
\newcommand{\mycommfont}[1]{{\scriptsize\itshape\textcolor{OliveGreen}{#1}}}

\newcommand{\funccommd}[1]{{\footnotesize\textcolor{RoyalBlue}{#1}}}

\newcommand{\clientcommand}[1]{{\footnotesize\textcolor{BrickRed}{#1}}}

\begin{algorithm}
\caption{\fluid executing on Centralized Server}
\label{alg:fluid}
\footnotesize


\begin{algorithmic}[1] %[1] enables line numbers

\STATE \textbf{Input}: $M(w)$ \quad \quad \mycommfont{\# Model}
\STATE \textbf{Output}: $S(w)$ \quad \quad \mycommfont{\# Sub-models for stragglers}
\\
\STATE $N$ $\rightarrow$ All Clients, $T$ $\rightarrow$ $\emptyset$ \quad \quad\mycommfont{\# T stragglers, N non-stragglers}
\STATE $M(w_0)$ = $Initial Model$ \quad \quad \mycommfont{\# Model with Weights at time=0}
\STATE $IN$ $\rightarrow$ $\emptyset$ \quad \quad\mycommfont{\# invariant neurons}
\STATE $done$ = FALSE  \quad \quad \mycommfont{\# flag to check if training done}
\\
\WHILE{not done}

\IF [\mycommfont{\# Straggler and dropout threshold intialization}]{$T$ is $\emptyset$}
\STATE \clientcommand{Broadcast} $M(w_0)$ to each $C$
\STATE \clientcommand{Receive} $M(w_{1})$ from every $C$
\STATE $th$ =  \funccommd{min} ($\frac{w_{ijct} - w_{ij(t-1)}}{w_{ij(t-1)}})$ \mycommfont{\# threshold for Invariant dropout}

\ELSE [\mycommfont{\# Straggler and dropout threshold recalibration}]
\STATE $S(w_t)$ = \funccommd{sub\_model\_generation}($inv$, $M(w_t)$) 
\STATE \clientcommand{Broadcast}  $S(w_{ti})$ all $i$ $\in$ $T$
\STATE \clientcommand{Broadcast} $M(w_t)$ all $i$ $\land \notin  T$
\STATE \clientcommand{Receive} $\Delta(w_{t+1})$ from every $C$

\STATE $M(w_{t+1})$ = \funccommd{aggregate}($M(w_t)$, $\Delta(w_{t+1})$)
\STATE $IN$ = \funccommd{identify\_invariant\_neurons}($th$,$\Delta(w_{t+1})$, $N$)

\ENDIF
\STATE $T$, $N$,$L$ = \funccommd{determine\_stragglers}($C$)  \mycommfont{\# $L$ = train latencies} 

\STATE $T_{target}$ = \funccommd{identify\_next\_slowest\_client}($L$)

\STATE $Speedup_i$ = $\frac{T_{straggler_i}}{T_{target}}$
\STATE $r_i$, $S_i$ = \funccommd{calculate\_submodel\_size}(${Speedup_i}$) \mycommfont{\# $r_i$ dropout rate} 
\STATE $th$ = \funccommd{increment\_threshold}($r_i$)

\STATE done = \funccommd{check\_training\_done}($M(w_t$))


\ENDWHILE

\end{algorithmic}
\end{algorithm}

==> body/tables/alpha_accuracy.tex <==
\begin{table*}[h!]
\centering
\caption{Effect of Slipstream parameter $\alpha$ on test accuracy}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c}
 \hline
 \textbf{$\alpha$} & \textbf{DLRM} & \textbf{$\alpha$ = 0} & \textbf{$\alpha$ = 4} & \textbf{$\alpha$ = 8} & \textbf{$\alpha$ =12} & \textbf{$\alpha$ = 16} & \textbf{$\alpha$ = 20} & \textbf{$\alpha$ = 24} &
 \textbf{$\alpha$ = 26}  \\ 
 \hline
 RM1 (Taobao) & 89.63\%	& 83.39\% & 88.37\%	& N/A & N/A	& N/A &	N/A	& N/A & N/A	 \\
 \hline
 RM2 (Criteo Kaggle) & 78.63\% &	77.78\%	& 78.4\%  & 78.56\%	& 78.59\%	& 78.59\% &	78.6\%	& 78.55\% & 78.59\%	 \\
 \hline
 RM3 (Criteo Terabyte) & 81.16\%	& 80.68\% &	81.02\%	& 81.01\%	& 81.04\%	& 81.01\% &	81.03\%	& 81.03\% & 81.16\% \\
 \hline
 RM4 (Avazu) & 83.59\% & 83.49\% & 83.49\% &	83.50\%	& 83.43\% & 83.51\%	& 83.49\% & N/A	& N/A	      \\
 \hline
\end{tabular}}
\label{tab:alpha1}
\end{table*}

==> body/tables/challenge1.tex <==
\begin{table}[h!]
\centering
\caption{Embedding Table Footprint and Size}
\resizebox{0.35\columnwidth}{!}{
\begin{tabular}{|c|c|c|}
 \hline
 \textbf{Model} & \textbf{Footprint} & \textbf{\# Rows}  \\
 & &  (Biggest Table) \\
 \hline
 RM1 & 0.3~GB & 4.1~Million\\
 RM2 & 2~GB & 10.1~Million \\
 RM3 & 63~GB & 11.9~Million\\
 RM4 & 0.55~GB & 6.6~Million\\
 \hline
\end{tabular}}
\label{tab:challenge1}
\end{table}

==> body/tables/challenge2.tex <==
\begin{table}[h!]
\centering
\caption{Accuracy drop from skipping Non-Popular Embeddings}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
 \hline
 \textbf{Dataset} & \textbf{Baseline} & \textbf{Skipping Non-Popular Embeddings} & \textbf{Difference}  \\
 \hline
 & & & & \hline
\end{tabular}}
\label{tab:challenge2}
\end{table}

==> body/tables/lambda.tex <==
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
 \textbf{$\Lambda$} & \textbf{$10^{-1}$} & \textbf{$10^{-2}$} & \textbf{$10^{-3}$} & \textbf{$10^{-4}$} & \textbf{$10^{-5}$} & \textbf{$10^{-6}$} & \textbf{$10^{-7}$} \\ 
 \hline
 RM1 (Taobao) & 0\%  & 0\% & 0\% & 1.03\% & 27.12\% 
 & 92.46\% & 100\% \\
 \hline
 RM2 (Criteo Kaggle) & 2.50\% & 24.12\% & 50.42\% & 65.11\% &
 75.83\% & 100\% & 100\& \\
 \hline
 RM3 (Criteo Terabyte) & 2.55\% & 23.63\% & 52.56\% & 73.06\% & 81.66\% & 100\% & 100\% \\
 \hline
 RM4 (Avazu) & 3.33\% &  8.88\% & 21.42\% & 44.16\% & 74.63\% & 100\%  & 100\%      \\
 \hline
\end{tabular}}
